Confined Electromagnetic Waves in Media Composed of Topological Insulators

Topological insulators (TIs) are quantum materials combining insulating bulk properties with conductive surface states protected by time-reversal symmetry. Their unique electromagnetic behavior originates from the topological magnetoelectric effect encoded in an axion-like $\theta$-term ($\theta$ = $\pi$ mod 2$\pi$). This $\theta$-electrodynamics modifies Maxwell's equations specifically at material interfaces through altered boundary conditions, preserving conventional bulk electrodynamics while enabling surface-mediated optical effects like polarization rotation and hybrid wave modes. This thesis explores electromagnetic wave confinement in TI-based waveguides. Key advances include: (1) Controlled modification of reactive and dissipated energies through polarization engineering in waveguide geometries; (2) Experimental realization of transverse electromagnetic (TEM) waves violating Earnshaw's theorem via $\theta$ discontinuities in coaxial TI structures, demonstrating unique polarization rotation mechanisms and low-loss propagation through bent fibers; (3) TEM wave confinement with fewer than two conductors using imaginary $\theta$ parameters, explained through self-consistent surface charge dynamics; (4) First-principles identification of hybrid TE-TM modes in TI slab waveguides, contrasting with conventional magnetoelectric material responses. These findings establish how surface boundary condition modifications from $\theta$ enable new electromagnetic solutions despite unchanged bulk equations. The demonstrated phenomena -- including modified propagation modes, non-trivial polarization dynamics, and unconventional confinement -- suggest photonic applications in polarization control and optical routing. By connecting topological electrodynamics with waveguide physics, this work provides both fundamental insights and practical design principles for topological photonic systems.

==> Otros/Calificaciones.tex <==
%Las calificaciones entregan la misma información de la portada y se le agrega la nota y la firma. Esta página es opcional.
\begin{titlepage}
	
	\newgeometry{top=1 in, bottom=1 in, left=1 in, right= 1 in} 
	
	\thispagestyle{frontpage}
	
	\begin{center}
		
		\vspace*{4\baselineskip}
	
		
		{\Huge \textbf{TÍTULO PRINCIPAL\\}}%No abreviar, no subrayar, no usar comillas. Se escribe completamente en mayúsculas
		        \vspace*{1.5\baselineskip}

		\large{\textit{subtítulo}}\\ %No abreviar, no subrayar, no usar comillas. Solo la priemra letra usa mayúsculas
		
        \vspace*{1,5\baselineskip}

		\large{\textbf{Por: Autor}}\\ %Nombre como aparece en registro académico
		
		\vspace{1,5\baselineskip}
		
		\large{Tesis presentada a la Facultad de Ciencias Físicas y Matemáticas de la Univerisdad de Concepción para optar al grado académico de Magister en Ciencias con Mención en Física.} %Cambiar a grado académico correspondiente. 
		
		\vspace{1,5\baselineskip}
		Diciembre 2019\\ %Mes y año de la tesis, solo primera letra del mes en mayúsculas
		Concepción, Chile %Ciudad y país de publicación.
\vspace{1,5\baselineskip}

		\large{\textbf{Profesor Guía: Nombre}}\\ %Nombre del profesor que dirigió el trabajo, de la comisión informante y otros asesores precedidos por los títulos correctos de la unidad académica.  
		%Al margen derecho del profesor guía se estampa la firma y/o calificación.
		

	\end{center}
	

	
\end{titlepage}

==> Otros/Dedicatoria.tex <==
%La dedicatoria debe ser ubicada en el extremo inferior derecho de una página vacía, está página es opcional
\thispagestyle{empty}
\begin{flushright}
\vfill
%\textit{
%Now the world can be an unfair place at times\\
%But your lows will have their compliment of highs\\
%And if anyone should cheat you\\
%Take advantage of or beat you raise your head\\
%And wear your wounds with pride.}
\vfill
\end{flushright}%Escribir aquí la dedicatoria

